Error Bounds and Guidelines for Privacy Calibration in Differentially Private Kalman Filtering

Differential privacy has emerged as a formal framework for protecting sensitive information in control systems. One key feature is that it is immune to post-processing, which means that arbitrary post-hoc computations can be performed on privatized data without weakening differential privacy. It is therefore common to filter private data streams. To characterize this setup, in this paper we present error and entropy bounds for Kalman filtering differentially private state trajectories. We consider systems in which an output trajectory is privatized in order to protect the state trajectory that produced it. We provide bounds on a priori and a posteriori error and differential entropy of a Kalman filter which is processing the privatized output trajectories. Using the error bounds we develop, we then provide guidelines to calibrate privacy levels in order to keep filter error within pre-specified bounds. Simulation results are presented to demonstrate these developments.

==> MultiAgent.tex <==
\section{Multi-Agent Setup}\label{sec:multiAgent}

In this section, we investigate the impact of providing differential privacy upon a network of agents in aggregate. We consider a collection of $N$ agents. The state trajectory of each agent is sensitive, and therefore it needs to be protected. We set ${ n =\sum_{i=1}^{N}n_i }$, which is the dimension of all agents' states in aggregate. 
We then concatenate the states of all agents within the network into the network-level state $x(k) = (x_1^T(k)\dots x_N^T(k) )^T \in \mathbb{R}^n$. Additionally, for the forthcoming analyses, we define network-level state dynamics to evolve according to 
\begin{align}
x(k+1) & = Hx(k)+w(k)\\
y(k) & = C x(k),
\end{align}
where $ w(k) = (w_1(k)^T, \dots ,w_N(k)^T) \in \mathbb{R}^n$, $ H = \diag (H_1, \dots , H_N)\in \mathbb{R}^{n\times n} $, and $ C= \diag (C_1, \dots , C_N)\in \mathbb{R}^{n\times q}$.
	





 




==> keywords.tex <==
\begin{IEEEkeywords}
	Differential Privacy, LQR, LQG, Privacy in Feedback, (what else?)
\end{IEEEkeywords}
